Backward martingale transport maps and equilibrium with insider

We consider an optimal transport problem with backward martingale constraint. The objective function is given by the scalar product of a pseudo-Euclidean space $S$. We show that the supremums over maps and plans coincide, provided that the law $\nu$ of the input random variable $Y$ is atomless. An optimal map $X$ exists if $\nu$ does not charge any $c-c$ surface (the graph of a difference of convex functions) with strictly positive normal vectors in the sense of the $S$-space. The optimal map $X$ is unique if $\nu$ does not charge $c-c$ surfaces with nonnegative normal vectors in the $S$-space. As an application, we derive sharp conditions for the existence and uniqueness of equilibrium in a multi-asset version of the model with insider from Rochet and Vila [10]. In the linear-Gaussian case, we characterize Kyle's lambda, the sensitivity of price to trading volume, as the unique positive solution of a non-symmetric algebraic Riccati equation.

==> style.tex <==
% Packages

\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage[numbers]{natbib}
\usepackage{tikz}
\usepackage{pgfplots}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section]
\newtheorem{Corollary}[Theorem]{Corollary}
\newtheorem{Lemma}[Theorem]{Lemma}
\newtheorem{Proposition}[Theorem]{Proposition}
\newtheorem{Claim}{Claim}

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}
\newtheorem{Definition}[Theorem]{Definition}
\newtheorem{Example}[Theorem]{Example}

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark}
\newtheorem{Problem}[Theorem]{Problem}

% Useful commands

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\as}[1]{#1-a.s.}
\newcommand{\braces}[1]{\left\lbrace{#1}\right\rbrace}
\newcommand{\cbraces}[1]{\left({#1}\right)} % curved braces around
\newcommand{\cord}{\prec_{\text{conv}}}
\newcommand{\descr}[2]{\braces{{#1}\;|\; #2}}
\newcommand{\cdescr}[2]{\cbraces{{#1}\;|\; #2}}
\newcommand{\diag}[1]{\mathrm{diag}(#1)}
\newcommand{\law}[1]{\Law(#1)}
\newcommand{\proj}[2]{\operatorname{proj}\nolimits_{#1}{#2}}
\newcommand{\seq}[1]{$\left(#1^n\right)_{n\geq 1}$}
\newcommand{\set}{:=}
\newcommand{\ip}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\ind}[1]{1_{\braces{#1}}}
\newcommand{\setind}[1]{1_{#1}}
\newcommand{\lsp}[2]{{\mathcal{L}_{#1}\cbraces{\real{#2}}}}
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain,
                                %3=val_domain                                
\newcommand{\mmap}[3]{#1:\; #2 \rightrightarrows #3} %1=name, 2=arg_domain,
                                %3=val_domain                               
\newcommand{\mset}[1]{\mathfrak{M}\cbraces{#1}} % maximal monotone set
\newcommand{\msym}[2]{\mathcal{S}^{#1}_{#2}} % symmetric dxd matrices
                                % with m positive eigenvalues
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\ps}[2]{\mathcal{P}_{#1}\cbraces{#2}} %probability space
\newcommand{\real}[1]{\mathbb{R}^{#1}}
\newcommand{\realext}{\mathbb{R} \cup \braces{+\infty}}
\newcommand{\realextminus}{\mathbb{R} \cup \braces{-\infty}}
\newcommand{\realextplusminus}{\mathbb{R} \cup \braces{-\infty} \cup \braces{+\infty}}
\newcommand{\pf}[2]{{#1}_{\#}{#2}}
\newcommand{\bpf}[2]{\cbraces{{#1}_{\#}{#2}}}

% Conditional expectation: measure, time, 
\newcommand{\cEP}[2]{\mathbb{E}\left(\left.#1\right\lvert{#2}\right)}
\newcommand{\EP}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\PP}[1]{\mathbb{P}\left({#1}\right)}
\newcommand{\cov}[3]{\Cov_{#1}(#2,#3)} %1=measure, 2=first rv,
                                %3=second rv.
\newcommand{\ccov}[4]{\Cov_{#1}(#2,#3|#4)} %1=measure, 2=first rv,
                                %3=second rv, #4 condition

% Operators

\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator*{\argmax}{arg\:max}
\DeclareMathOperator*{\argmin}{arg\:min}
\DeclareMathOperator{\boundary}{\partial}
\DeclareMathOperator*{\clconv}{\cl{\conv}}
\DeclareMathOperator*{\cl}{cl}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator*{\esssup}{ess\:sup}
\DeclareMathOperator*{\essinf}{ess\:inf}
\DeclareMathOperator*{\image}{image}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\kernel}{kernel}
\DeclareMathOperator*{\ri}{ri}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\range}{range}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Law}{{Law}}


